On Allocation Policies for Power and Performance

With the increasing popularity of Internet-based services and applications, power efficiency is becoming a major concern for data center operators, as high electricity consumption not only increases greenhouse gas emissions, but also increases the cost of running the server farm itself. In this paper we address the problem of maximizing the revenue of a service provider by means of dynamic allocation policies that run the minimum amount of servers necessary to meet user's requirements in terms of performance. The results of several experiments executed using Wikipedia traces are described, showing that the proposed schemes work well, even if the workload is non-stationary. Since any resource allocation policy requires the use of forecasting mechanisms, various schemes allowing compensating errors in the load forecasts are presented and evaluated.

==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

% \todo[inline]{Is this section still needed? If yes, it needs an update}

In this paper we have introduced and evaluated some easily implementable
policies for dynamically adaptable Internet services. 

Under some simplifying assumptions, the
numerical algorithm implemented by the `Adaptive' policy can find the
best trade off between consumed power and delivered service quality, while the
QED heuristic we have introduced performs well. A special focus has been given
to issues related to the quality of the workload estimation ({\it i.e.}, predicting the future arrival
rate). The enhancement adressing the latter problem were suggested and evaluated using Wikipedia traces, showing significant improvements over the original policies which assume that the parameters are known and accurate.


\section*{Acknowledgements}

The authors would like to thank the EU Cost Action IC0804 (Energy Efficiency
in Large Scale Distributed Systems), and the EUREKA
Project 4989 (SITIO).

%This work was partly funded by the European 
%Commission under the Seventh Framework Programme through the SEARCHiN project 
%(Marie Curie Action, contract number FP6-042467). 
%The authors would also like to thank EU Cost Action IC0804 (Energy Efficiency
%in Large Scale Distributed Systems).


==> future_work.tex <==
\section{Future Work}
\label{sec:future_work}

In this paper we have evaluated the performance of the proposed policies via simulation. Next, 
we plan to expand this work by implementing a prototype mimicking 
Wikipedia setup with real servers. 

% In our past work~\cite{mazzucco:2010a} we studied the impact of the 
% quality of the forecasting tools on the revenue, energy consumption, 
% etc. However, in order to evaluate the possible outcomes from deploying 
% the presented approaches one needs to know the quality of the forecasting 
% tools.  
% In the future work we plan to apply more advanced forecasting tool 
% such as ARIMA in order to predict the workloads and evaluate their
% efficiency for example with Wikipedia traces.  

Our model is currently designed to optimize the energy consumption
of a single tiered system. However, a significant percentage of
systems is implemented as two or three tiered, where one tier can be 
used for realizing caching, the second hosts application logic 
and the third is responsible for accommodating database servers.  
Thus, we plan to deal with scenarios where more than one tier is used. Also, we plan to assess the performance of the proposed policies under different workloads ({\it e.g.}, compute intensive, communication intensive and storage intensive).

Other issues we plan to deal with include electricity charges and PUE factor.
Currently we assume that the service provider is charged a flat fee for electricity consumption. 
However, when it comes to purchasing electricity in large amounts 
the price fluctuates depending on the time of the day, day of the week,
{\it etc}. Factoring in dynamic prices for electricity constitutes another 
direction of the future development of this work.   
Finally, depending on the size and type of the data center different cooling 
systems can be employed. 
Elaborating the model in order to incorporate the cooling costs depending
on the type of the cooling system is another possible future direction.


==> introduction.tex <==
%\todo[inline, color=green]{Abstract is missing}

\section{Introduction}
\label{sec:introduction}

 
A server farm is a collection of servers interconnected by high-speed, switched
LANs that hosts content and runs applications (or services) accessed over the
Internet. Data centers are an attractive alternative to enterprise systems
because they offer economies of scale for network, power, cooling,
administration, security and surge capacity~\cite{chase:2001}. However, because
of the high users' expectations in terms of performance~\cite{linder:2006a,
shankland:2008}, operating server farms in an energy efficient way is a
challenging problem as service providers operate under
stringent performance requirements, no matter whether they are dictated by users (see~\cite{jung:2009}
and the references cited therein) or by Service Level Agreements (SLAs). At the
moment, most of data center operators perform try to optimize their computational facilities for performance while ignoring energy consumption factors. 
However, given that the cost of servers purchase is comparable with the cost of the electricity required to run them for a 3 years period, power efficiency is becoming one of the major
concerns for service providers, as it markedly affects the cost of running
the data centers themselves. 
Consequently, it is of great importance to develop
strategies aiming at reducing the power consumption while maintaining acceptable levels of performance.

While different techniques can be employed to reduce the server farm energy
requirements (see Section~\ref{sec:related_work} for more details), most of
the efforts focus on single and specific architectural and technological
improvements for achieving power reduction, ignoring the fact that power
efficiency as a ratio of performance to power consumption is affected by both
performance improvements and power reduction~\cite{gruber:2010}. 
Hence, the only way to
\emph{significantly} reduce data centers' power consumption is to improve the
server farm's utilization, {\it e.g.}, by tearing down servers in excess. The
model we propose takes into account the fact that users are impatient and that
servers energy consumption depends on servers' utilization. Therefore, we
study and evaluate dynamic allocation policies aiming at maximizing the overall
performance while minimizing the number of required servers when the traffic parameters are \emph{not} known. 
 
 Next, we discuss how server farms can be designed and operated, and introduce the system model.
 Then we describe the model of user demand and service provision we propose, and present various energy aware allocation policies (Section~\ref{sec:policies}).
 Section~\ref{sec:experiments} contains several experiments we have carried out using the Wikipedia traces, while a survey of relevant related work is presented in Section~\ref{sec:related_work}. Finally, we conclude the paper with future work and some remarks.
 



==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

As large scale distributed systems gather and share more and more computing 
nodes and storage resources their energy consumption rises very quickly.
 On the other hand, in order to make a fully efficient use of computing and
 communication systems and reduce their environmental and social impact, green
 computing and communication research has increasingly become a hot topic of 
 interest for both the computer research community and industry.
Unfortunately, while the problem of energy
efficiency in mobile devices and laptops has already attracted a lot of
attention, the problem of energy efficiency in data centers remains under
researched. All the efforts in this area are either $(i)$~intensive, {\it i.e.},
optimizing power consumption of a server, for example by dynamically changing the
CPU voltage/frequency, or $(ii)$~extensive, {\it i.e.}, minimizing the power
consumption of a server pool, for example by dynamically switching some servers
off when they are not needed,

%Intensive
Most of the intensive approaches have tried to minimize the
power consumption when the number of servers is fixed. 
While Google engineers have called for systems designers to develop servers 
that consume energy in proportion to the amount of computing work they 
perform~\cite{barroso:2007} and Microsoft engineers have been working on 
better power management on the operating system layer~\cite{microsoft:2009}, 
the reality is that servers consume as much as 65\% of their peak power  when
idle~\cite{greenberg:2009}. 
Hence, Elnozahy et al.~\cite{Elnozahy:2002} investigated
the potential benefits of scaling down the CPU voltage/frequency according to the offered
load, finding that savings can be as big as 20--29\%, while Wierman et al.~\cite{wierman:2009} and Horvath et el.~\cite{Horvath:2007} considered
changing the voltage of servers' CPU in order to minimize the power consumption while trying to meet certain predefined deadlines. 

% Extensive
Most of the research conducted using extensive methodologies considered
scenarios where the number of running servers can be controlled at runtime. 
Thus, the idea is to power 
down some servers whenever that can be justified by demand conditions. 
For example, Chase et al.~\cite{chase:2001} presented an 
architecture for resource management of server farms. There the goal is to 
reduce energy consumption, while the SLAs are assumed to be flexible ({\it
i.e.}, service degradation is a viable option). 
The most closely related work can perhaps be found in~\cite{chen:2005}
and~\cite{mazzucco:2010a}. \cite{chen:2005} presents a queuing model
for controlling the energy consumption of service provisioning systems subject to Service Level
Agreements (SLAs). However, while Chen et al. take into account the cost for
smaller mean time between failures (MTBF) when powering up/down some servers, the cost function they
propose does not consider the time and energy wasted during state changes, nor
the cost for failing to meet the promised quality requirements. Hence, the taken
decisions could be
either too performance oriented or too energy-efficiency oriented. 
\cite{mazzucco:2010a}, instead, discusses a problem similar to that we attack in
this paper. However, in that paper the authors assume that clients have no
patience, while they do not consider the fact that servers consume energy
without producing any revenue during system reconfigurations. 


Finally, since running too many servers increases the electricity consumption
while having too few servers switched on requires running
those servers' CPUs at higher frequencies, some hybrid approaches have been
proposed. For example,~\cite{Elnozahy:2002} attempts to
find a rational trade off between the number of servers switched on and the voltage/frequency of the CPU on each server.

%\todo[inline]{
%D: I would say that  

%Besides, because of several reasons, including risk management and uncertainty in demand forecast, the resource utilization of server farms is rather poor (the typical CPU utilization ranges between 15\% and 35\%~\cite{hamilton:2008}, while the utilization of any resource in excess of 50\% occurs very rarely~\cite{stewart:2007}).
%}

